Adaptive FEM with explicit time integration for the wave equation

Starting from a recent a posteriori error estimator for the finite element solution of the wave equation with explicit time-stepping [Grote, Lakkis, Santos, 2024], we devise a space-time adaptive strategy which includes both time evolving meshes and local time-stepping [Diaz, Grote, 2009] to overcome any overly stringent CFL stability restriction on the time-step due to local mesh refinement. Moreover, at each time-step the adaptive algorithm monitors the accuracy thanks to the error indicators and recomputes the current step on a refined mesh until the desired tolerance is met; meanwhile, the mesh is coarsened in regions of smaller errors. Leapfrog based local time-stepping is applied in all regions of local mesh refinement to incorporate adaptivity into fully explicit time integration with mesh change while retaining efficiency. Numerical results illustrate the optimal rate of convergence of the a posteriori error estimators on time evolving meshes.

==> alfafem.tex <==

@article{ZankSteinbach:16:article:Adaptive-Space-Time,
	author = {Zank, Marco and Steinbach, Olaf},
	doi = {10.1002/pamm.201610377},
	issn = {1617-7061},
	journal = {PAMM},
	number = {1},
	pages = {777--778},
	title = {Adaptive Space-Time Boundary Element Methods for the Wave Equation},
	volume = {16},
	year = {2016}}


@article{BignardiMoiola:25:article:A-Space--Time-Continuous,
	abstract = {We propose a new space--time variational formulation for wave equation initial--boundary value problems. The key property is that the formulation is coercive (sign-definite) and continuous in a norm stronger than \$\$H\textasciicircum 1(Q)\$\$, Q being the space--time cylinder. Coercivity holds for constant-coefficient impedance cavity problems posed in star-shaped domains, and for a class of impedance--Dirichlet problems. The formulation is defined using simple Morawetz multipliers and its coercivity is proved with elementary analytical tools, following earlier work on the Helmholtz equation. The formulation can be stably discretised with any \$\$H\textasciicircum 2(Q)\$\$-conforming discrete space, leading to quasi-optimal space--time Galerkin schemes. Several numerical experiments show the excellent properties of the method.},
	author = {Bignardi, Paolo and Moiola, Andrea},
	date-added = {2025-12-09 09:45:30 +0000},
	date-modified = {2025-12-09 11:49:35 +0000},
	doi = {10.1007/s00211-025-01478-3},
	issn = {0945-3245},
	journal = {Numerische Mathematik},
	keywords = {35L05,65M15,65M60},
	langid = {english},
	month = aug,
	number = {4},
	pages = {1211--1258},
	title = {A Space--Time Continuous and Coercive Formulation for the Wave Equation},
	volume = {157},
	year = 2025}


@techreport{DongGeorgoulisMascottoWang:25:techreport:A-Posteriori-Error,
	author = {Dong, Zhaonan and Georgoulis, Emmanuil H. and Mascotto, Lorenzo and Wang, Zuodong},
	doi = {10.48550/arXiv.2509.08537},
	eprint = {2509.08537},
	howpublished = {online preprint},
	institution = {arXiv},
	month = 09,
	number = {arXiv:2509.08537},
	publisher = {arXiv},
	title = {A Posteriori Error Analysis and Adaptivity of a Space-Time Finite Element Method for the Wave Equation in Second Order Formulation},
	year = 2025}


@article{BangerthGroteHohenegger:04:article, 
author = {Bangerth, W. and Grote, M. J. and Hohenegger, C.},
title =  {Finite Element Method for Time Dependent Scattering: Nonreflecting Boundary 
Conditions, Adaptivity, and Energy Decay},
journal = {Comp. Meth. Appl. Mech. Engrg.},
volume = {193}, 
year = {2004},
pages = {2453--2482}
}

@article{Skeel:93:article, 
author = {Skeel, R. D. },
title =  {Variable step size destabilizes the
St\"ormer/Leapfrog/Verlet method},
journal = {BIT},
volume = {33}, 
year = {1993},
pages = {172--175}
}

@article{ThompsonHe:05:article, 
author = {Thompson, L. L. and He, D.},
title =  {Adaptive space–time finite element methods for the
wave equation on unbounded domains},
journal = {Comp. Meth. Appl. Mech. Engrg.},
volume = {194}, 
year = {2005},
pages = {1947--2000}
}


@article{DiazGrote:09:article:Energy-Conserving,
  author =        {Diaz, J. and Grote, M. J.},
  journal =       {SIAM Journal on Scientific Computing},
  month =         {01},
  number =        {3},
  pages =         {1985--2014},
  publisher =     {{Society for Industrial and Applied Mathematics}},
  title =         {Energy Conserving Explicit Local Time Stepping for
                   Second-Order Wave Equations},
  volume =        {31},
  year =          {2009},
  abstract =      {Locally refined meshes severely impede the efficiency
                   of explicit Runge--Kutta (RK) methods for the
                   simulation of time-dependent wave phenomena. By
                   taking smaller time-steps precisely where the
                   smallest elements are located, local time-stepping
                   (LTS) methods overcome the bottleneck caused by the
                   stringent stability constraint of but a few small
                   elements in the mesh. Starting from classical or
                   low-storage explicit RK methods, explicit LTS methods
                   of arbitrarily high accuracy are derived. When
                   combined with an essentially diagonal finite element
                   mass matrix, the resulting time-marching schemes
                   retain the high accuracy, stability, and efficiency
                   of the original RK methods while circumventing the
                   geometry-induced stiffness. Numerical experiments
                   with continuous and discontinuous Galerkin finite
                   element discretizations corroborate the expected
                   rates of convergence and illustrate the usefulness of
                   these LTS-RK methods.},
  doi =           {10.1137/070709414},
  issn =          {1064-8275},
}


@book{AinsworthOden:00:book:A-posteriori,
  address =       {New York},
  author =        {Ainsworth, M. and Oden, J. Tinsley},
  pages =         {xx+240},
  publisher =     {Wiley-Interscience [John Wiley \& Sons]},
  series =        {Pure and Applied Mathematics (New York)},
  title =         {A posteriori error estimation in finite element
                   analysis},
  year =          {2000},
  isbn =          {0-471-29411-X},
  url =           {http://www.worldcat.org/oclc/61130479},
}

@book{Verfurth:13:book:A-posteriori,
  author =        {Verf{\"u}rth, R.},
  publisher =     {Oxford University Press, Oxford},
  series =        {Numerical {Mathematics} and {Scientific}
                   {Computation}},
  title =         {A posteriori error estimation techniques for finite
                   element methods},
  year =          {2013},
  doi =           {10.1093/acprof:oso/9780199679423.001.0001},
  isbn =          {978-0-19-967942-3},
  url =           {http://www.worldcat.org/oclc/5564393801},
}

@article{Verfurth:03:article:A-posteriori,
	author = {Verf{\"u}rth, R.},
	date-added = {2013-06-19 16:13:51 +0100},
	date-modified = {2019-06-25 09:51:53 +0100},
	doi = {10.1007/s10092-003-0073-2},
	fjournal = {Calcolo. A Quarterly on Numerical Analysis and Theory of Computation},
	issn = {0008-0624},
	journal = {Calcolo},
	mrclass = {65M60 (65M15)},
	mrnumber = {2025602 (2005f:65131)},
	number = {3},
	pages = {195--212},
	title = {A posteriori error estimates for finite element discretizations of the heat equation},
	url = {https://doi.org/10.1007/s10092-003-0073-2},
	volume = {40},
	year = {2003},
	bdsk-file-1 = {YnBsaXN0MDDSAQIDBFxyZWxhdGl2ZVBhdGhYYm9va21hcmtvEEYALgAuAC8ALgAuAC8ATABpAHQAZQByAGEAdAB1AHIAZQAvAEEAdQB0AGgAbwByAC8AVgAvAFYAZQAvAFYAZQByAGYAdQMIAHIAdABoAC0AMgAwADAAMwAtAGEAcgB0AGkAYwBsAGUALQBBAC0AQQAgAHAAbwBzAHQAZQByAGkAbwByAGkALgBwAGQAZk8RBHRib29rdAQAAAAABBAwAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAABwAwAABQAAAAEBAABVc2VycwAAAAQAAAABAQAAb2wyMAcAAAABAQAARHJvcGJveAAKAAAAAQEAAExpdGVyYXR1cmUAAAYAAAABAQAAQXV0aG9yAAABAAAAAQEAAFYAAAACAAAAAQEAAFZlAAAqAAAAAQEAAFZlcmZ1zIhydGgtMjAwMy1hcnRpY2xlLUEtQSBwb3N0ZXJpb3JpLnBkZgAAIAAAAAEGAAAEAAAAFAAAACAAAAAwAAAARAAAAFQAAABgAAAAbAAAAAgAAAAEAwAA61wAAAAAAAAIAAAABAMAABRvBAAAAAAACAAAAAQDAACl4igAAAAAAAgAAAAEAwAAQ+UoAAAAAAAIAAAABAMAAEjmKAAAAAAACAAAAAQDAABx6igAAAAAAAgAAAAEAwAATvEoAAAAAAAIAAAABAMAAK2hKwAAAAAAIAAAAAEGAADIAAAA2AAAAOgAAAD4AAAACAEAABgBAAAoAQAAOAEAAAgAAAAABAAAQbBuvO4AAAAYAAAAAQIAAAEAAAAAAAAADwAAAAAAAAAAAAAAAAAAAAgAAAAEAwAABgAAAAAAAAAEAAAAAwMAAOQUAAAIAAAAAQkAAGZpbGU6Ly8vDAAAAAEBAABNYWNpbnRvc2ggSEQIAAAABAMAAACQgpbnAAAACAAAAAAEAABBxrzVhQAAACQAAAABAQAAM0VBNUY0MzQtNEQ3OC00MUE0LUJENTctOTQxNTkxNTRDRjkxGAAAAAECAACBAAAAAQAAAO8TAAABAAAAAAAAAAAAAAABAAAAAQEAAC8AAAAAAAAAAQUAAAcBAAABAgAANmQ0ZDczMTJiODBmOWY2OGRlYjVjMzBmOTRmYmZiYmUxZGZjYWMxN2QxN2U2YWRhOWYyYTY1MDBmNDA4MjZiMTswMDswMDAwMDAwMDswMDAwMDAwMDswMDAwMDAwMDswMDAwMDAwMDAwMDAwMDIwO2NvbS5hcHBsZS5hcHAtc2FuZGJveC5yZWFkLXdyaXRlOzAxOzAxMDAwMDBmOzAwMDAwMDAwMDAyYmExYWQ7MDE7L3VzZXJzL29sMjAvZHJvcGJveC9saXRlcmF0dXJlL2F1dGhvci92L3ZlL3ZlcmZ1zIhydGgtMjAwMy1hcnRpY2xlLWEtYSBwb3N0ZXJpb3JpLnBkZgAAzAAAAP7///8BAAAAAAAAABAAAAAEEAAAoAAAAAAAAAAFEAAASAEAAAAAAAAQEAAAgAEAAAAAAABAEAAAcAEAAAAAAAACIAAATAIAAAAAAAAFIAAAvAEAAAAAAAAQIAAAzAEAAAAAAAARIAAAAAIAAAAAAAASIAAA4AEAAAAAAAATIAAA8AEAAAAAAAAgIAAALAIAAAAAAAAwIAAAWAIAAAAAAAABwAAAoAEAAAAAAAARwAAAFAAAAAAAAAASwAAAsAEAAAAAAACA8AAAYAIAAAAAAAAACAANABoAIwCyAAAAAAAAAgEAAAAAAAAABQAAAAAAAAAAAAAAAAAABSo=},
	bdsk-url-1 = {http://www.ams.org/mathscinet-getitem?mr=2025602},
	bdsk-url-2 = {http://dx.doi.org/10.1007/s10092-003-0073-2}}


@article{ErikssonJohnson:91:article:Adaptive,
  author =        {Eriksson, K. and Johnson, C.},
  journal =       {SIAM J. Numer. Anal.},
  number =        {1},
  pages =         {43--77},
  title =         {Adaptive finite element methods for parabolic
                   problems. {I}. {A} linear model problem},
  volume =        {28},
  year =          {1991},
  doi =           {10.1137/0728003},
  issn =          {0036-1429},
  url =           {https://doi.org/10.1137/0728003},
}

@article{Picasso:98:article:Adaptive,
  author =        {Picasso, M.},
  journal =       {Comput. Methods Appl. Mech. Engrg.},
  number =        {3-4},
  pages =         {223--237},
  title =         {Adaptive finite elements for a linear parabolic
                   problem},
  volume =        {167},
  year =          {1998},
  doi =           {10.1016/S0045-7825(98)00121-2},
  issn =          {0045-7825},
  url =           {http://dx.doi.org/10.1016/S0045-7825(98)00121-2},
}

@article{ChenJia:04:article:An-adaptive,
  author =        {Chen, Z. and Jia, F.},
  journal =       {Math. Comp.},
  number =        {247},
  pages =         {1167--1193 (electronic)},
  title =         {An adaptive finite element algorithm with reliable
                   and efficient error control for linear parabolic
                   problems},
  volume =        {73},
  year =          {2004},
  issn =          {0025-5718},
}

@article{GaspozSiebertKreuzerZiegler:19:article:A-convergent,
  author =        {Gaspoz, F. D. and Siebert, K. and
                   Kreuzer, C. and Ziegler, D. A.},
  journal =       {IMA Journal of Numerical Analysis},
  month =         {04},
  number =        {2},
  pages =         {650--686},
  title =         {A convergent time--space adaptive {dG}(s) finite
                   element method for parabolic problems motivated by
                   equal error distribution},
  volume =        {39},
  year =          {2019},
  abstract =      {Abstract. We shall develop a fully discrete
                   space-time adaptive method for linear parabolic
                   problems based on new, reliable and efficient a
                   posteriori analysis},
  doi =           {10.1093/imanum/dry005},
  issn =          {0272-4979},
  language =      {en},
  url =           {https://academic-oup-com.ezproxy.sussex.ac.uk/imajna/
                  article/39/2/650/4960122},
}

@article{Johnson:93:article:Discontinuous,
  author =        {Johnson, C.},
  journal =       {Comput. Methods Appl. Mech. Engrg.},
  number =        {1-2},
  pages =         {117--129},
  title =         {Discontinuous {G}alerkin finite element methods for
                   second order hyperbolic problems},
  volume =        {107},
  year =          {1993},
  doi =           {10.1016/0045-7825(93)90170-3},
  issn =          {0045-7825},
}

@article{HulbertHughes:90:article:Space-Time-Finite,
  author =        {Hulbert, G. M. and Hughes, T. J. R.},
  journal =       {Computer Methods in Applied Mechanics and
                   Engineering},
  month =         {12},
  number =        {3},
  pages =         {327--348},
  title =         {Space-Time Finite Element Methods for Second-Order
                   Hyperbolic Equations},
  volume =        {84},
  year =          {1990},
  abstract =      {Space-time finite element methods are presented to
                   accurately solve elastodynamics problems that include
                   sharp gradients due to propagating waves. The new
                   methodology involves finite element discretization of
                   the time domain as well as the usual finite element
                   discretization of the spatial domain. Linear
                   stabilizing mechanisms are included which do not
                   degrade the accuracy of the space-time finite element
                   formulation. Nonlinear discontinuity-capturing
                   operators are used which result in more accurate
                   capturing of steep fronts in transient solutions
                   while maintaining the high-order accuracy of the
                   underlying linear algorithm in smooth regions. The
                   space-time finite element method possesses a firm
                   mathematical foundation in that stability and
                   convergence of the method have been proved. In
                   addition, the formulation has been extended to
                   structural dynamics problems and can be extended to
                   higher-order hyperbolic systems.},
  doi =           {10.1016/0045-7825(90)90082-W},
  issn =          {0045-7825},
}

@article{BangerthRannacher:01:article:Adaptive,
  author =        {Bangerth, W. and Rannacher, R.},
  journal =       {J. Comput. Acoust.},
  number =        {2},
  pages =         {575--591},
  title =         {Adaptive finite element techniques for the acoustic
                   wave equation},
  volume =        {9},
  year =          {2001},
  doi =           {10.1142/S0218396X01000668},
  issn =          {0218-396X},
}

@article{BernardiSuli:05:article:Time,
  author =        {Bernardi, C. and S{\"u}li, E.},
  journal =       {Math. Models Methods Appl. Sci.},
  number =        {2},
  pages =         {199--225},
  title =         {Time and space adaptivity for the second-order wave
                   equation},
  volume =        {15},
  year =          {2005},
  annote =        {Strangely, it took forever to get a first paper for
                   aposteriori error estimates for the wave equation.
                   The estimates are quite standard in nature, for the
                   Euler (2-step) scheme.},
  doi =           {10.1142/S0218202505000339},
  issn =          {0218-2025},
}

@article{Adjerid:02:article:A-posteriori,
  author =        {Adjerid, S.},
  journal =       {Comput. Methods Appl. Mech. Engrg.},
  number =        {41-42},
  pages =         {4699--4719},
  title =         {A posteriori finite element error estimation for
                   second-order hyperbolic problems},
  volume =        {191},
  year =          {2002},
  doi =           {10.1016/S0045-7825(02)00400-0},
  issn =          {0045-7825},
}

@article{Adjerid:06:article:A-posteriori,
  author =        {Adjerid, S.},
  journal =       {Comput. Methods Appl. Mech. Engrg.},
  number =        {33-36},
  pages =         {4203--4219},
  title =         {A posteriori error estimation for the method of
                   lumped masses applied to second-order hyperbolic
                   problems},
  volume =        {195},
  year =          {2006},
  doi =           {10.1016/j.cma.2005.08.003},
  issn =          {0045-7825},
}

@article{Picasso:10:article:Numerical,
  author =        {Picasso, M.},
  journal =       {SIAM Journal on Scientific Computing},
  number =        {4},
  pages =         {2213-2234},
  publisher =     {SIAM},
  title =         {Numerical Study of an Anisotropic Error Estimator in
                   the $L^2(H^1)$ Norm for the Finite Element
                   Discretization of the Wave Equation},
  volume =        {32},
  year =          {2010},
  doi =           {10.1137/090778249},
}

@article{GoryninaLozinskiPicasso:19:article:An-Easily-Computable,
  author =        {Gorynina, O. and Lozinski, A. and Picasso, M.},
  journal =       {ESAIM: Mathematical Modelling and Numerical Analysis},
  month =         {05},
  number =        {3},
  pages =         {729--747},
  publisher =     {EDP Sciences},
  title =         {An Easily Computable Error Estimator in Space and
                   Time for the Wave Equation},
  volume =        {53},
  year =          {2019},
  abstract =      {We propose a cheaper version of \emph{a
                   posteriori{$<$}i/{$>$} error estimator from Gorynina
                   \emph{et al.{$<$}i/{$>$} (\emph{Numer.
                   Anal.{$<$}i/{$>$} (2017)) for the linear second-order
                   wave equation discretized by the Newmark scheme in
                   time and by the finite element method in space. The
                   new estimator preserves all the properties of the
                   previous one (reliability, optimality on smooth
                   solutions and quasi-uniform meshes) but no longer
                   requires an extra computation of the Laplacian of the
                   discrete solution on each time step.}}}},
  doi =           {10.1051/m2an/2018049},
  issn =          {0764-583X, 1290-3841},
}

@article{GeorgoulisLakkisMakridakisVirtanen:16:article:A-Posteriori,
  author =        {Georgoulis, E. H. and Lakkis, O. and
                   Makridakis, C. G. and Virtanen, J. M.},
  journal =       {SIAM Journal on Numerical Analysis},
  month =         {01},
  number =        {1},
  pages =         {120--136},
  title =         {A Posteriori Error Estimates for Leap-Frog and Cosine
                   Methods for Second Order Evolution Problems},
  volume =        {54},
  year =          {2016},
  abstract =      {We consider second order explicit and implicit
                   two-step time-discrete schemes for wave-type
                   equations. We derive optimal order a posteriori
                   estimates controlling the time discretization error.
                   Our analysis has been motivated by the need to
                   provide a posteriori estimates for the popular
                   leap-frog method (also known as Verlet's method in
                   the molecular dynamics literature); it is extended,
                   however, to general cosine-type second order methods.
                   The estimators are based on a novel reconstruction of
                   the time-dependent component of the approximation.
                   Numerical experiments confirm similarity of the
                   convergence rates of the proposed estimators and the
                   theoretical convergence rate of the true error.},
  doi =           {10.1137/140996318},
  issn =          {0036-1429},
  url =           {https://arxiv.org/abs/1411.7572},
}

@article{Dupont:82:article:Mesh,
  author =        {Dupont, T.},
  journal =       {Math. Comp.},
  number =        {159},
  pages =         {85--107},
  title =         {Mesh modification for evolution equations},
  volume =        {39},
  year =          {1982},
  issn =          {0025-5718},
}

@article{LakkisPryer:12:article:Gradient,
  author =        {Lakkis, O. and Pryer, T.},
  journal =       {IMA J. Numer. Anal.},
  number =        {1},
  pages =         {246--278},
  title =         {Gradient recovery in adaptive finite-element methods
                   for parabolic problems},
  volume =        {32},
  year =          {2012},
  doi =           {10.1093/imanum/drq019},
  issn =          {0272-4979},
}

@article{KarakashianMakridakis:05:article:Convergence,
  author =        {Karakashian, O. and Makridakis, C.},
  journal =       {Math. Comp.},
  number =        {249},
  pages =         {85--102 (electronic)},
  title =         {Convergence of a continuous {G}alerkin method with
                   mesh modification for nonlinear wave equations},
  volume =        {74},
  year =          {2005},
  doi =           {10.1090/S0025-5718-04-01654-0},
  issn =          {0025-5718},
}

@article{GroteMitkova:10:article:Explicit-Local,
  author =        {Grote, M. J. and Mitkova, T.},
  journal =       {Journal of Computational and Applied Mathematics},
  month =         {10},
  number =        {12},
  pages =         {3283--3302},
  title =         {Explicit Local Time-Stepping Methods for
                   {{Maxwell}}'s Equations},
  volume =        {234},
  year =          {2010},
  abstract =      {Explicit local time-stepping methods are derived for
                   time dependent Maxwell equations in conducting and
                   non-conducting media. By using smaller time steps
                   precisely where smaller elements in the mesh are
                   located, these methods overcome the bottleneck caused
                   by local mesh refinement in explicit time
                   integrators. When combined with a finite element
                   discretisation in space with an essentially diagonal
                   mass matrix, the resulting discrete time-marching
                   schemes are fully explicit and thus inherently
                   parallel. In a non-conducting source-free medium they
                   also conserve a discrete energy, which provides a
                   rigorous criterion for stability. Starting from the
                   standard leap-frog scheme, local time-stepping
                   methods of arbitrarily high accuracy are derived for
                   non-conducting media. Numerical experiments with a
                   discontinuous Galerkin discretisation in space
                   validate the theory and illustrate the usefulness of
                   the proposed time integration schemes.},
  doi =           {10.1016/j.cam.2010.04.028},
  issn =          {0377-0427},
}

@article{GroteMehlinSauter:18:article:Convergence,
  author =        {Grote, M. J. and Mehlin, M. and
                   Sauter, S. A.},
  journal =       {SIAM Journal on Numerical Analysis},
  month =         {01},
  number =        {2},
  pages =         {994--1021},
  title =         {Convergence Analysis of Energy Conserving Explicit
                   Local Time-Stepping Methods for the Wave Equation},
  volume =        {56},
  year =          {2018},
  abstract =      {Local adaptivity and mesh refinement are key to the
                   efficient simulation of wave phenomena in
                   heterogeneous media or complex geometry. Locally
                   refined meshes, however, dictate a small time step
                   everywhere with a crippling effect on any explicit
                   time-marching method. In [J. Diaz and M. J. Grote,
                   SIAM J. Sci. Comput., 31 (2009), pp. 1985--2014] a
                   leap-frog (LF)-based explicit local time-stepping
                   (LTS) method was proposed, which overcomes the severe
                   bottleneck due to a few small elements by taking
                   small time steps in the locally refined region and
                   larger steps elsewhere. Here optimal convergence
                   rates are rigorously proved for the fully discrete
                   LTS-LF method when combined with a standard
                   conforming finite element method (FEM) in space.
                   Numerical results further illustrate the usefulness
                   of the LTS-LF Galerkin FEM in the presence of corner
                   singularities.},
  doi =           {10.1137/17M1121925},
  issn =          {0036-1429},
}

@article{GroteMichelSauter:21:article:Stabilized,
  author =        {Grote, M. J. and Michel, S. and Sauter, S. A.},
  journal =       {Mathematics of Computation},
  month =         {11},
  number =        {332},
  pages =         {2603--2643},
  title =         {Stabilized leapfrog based local time-stepping method
                   for the wave equation},
  volume =        {90},
  year =          {2021},
  abstract =      {Local time-stepping methods permit to overcome the
                   severe stability constraint on explicit methods
                   caused by local mesh refinement without sacrificing
                   explicitness. Diaz and Grote [SIAM J. Sci. Comput. 31
                   (2009), pp. 1985--2014] proposed a leapfrog based
                   explicit local time-stepping (LF-LTS) method for the
                   time integration of second-order wave equations.
                   Recently, optimal convergence rates were proved for a
                   conforming FEM discretization, albeit under a CFL
                   stability condition where the global time-step,
                   Δ⁢t, depends on the smallest elements in the mesh
                   (see M. J. Grote, M. Mehlin, and S. A. Sauter [SIAM
                   J. Numer. Anal. 56 (2018), pp. 994--1021]). In
                   general one cannot improve upon that stability
                   constraint, as the LF-LTS method may become unstable
                   at certain discrete values of Δ⁢t. To remove those
                   critical values of Δ⁢t, we apply a slight
                   modification (as in recent work on LF-Chebyshev
                   methods by Carle, Hochbruck, and Sturm [SIAM J.
                   Numer. Anal. 58 (2020), pp. 2404--2433]) to the
                   original LF-LTS method which nonetheless preserves
                   its desirable properties: it is fully explicit,
                   second-order accurate, satisfies a three-term
                   (leapfrog like) recurrence relation, and conserves
                   the energy. The new stabilized LF-LTS method also
                   yields optimal convergence rates for a standard
                   conforming FE discretization, yet under a CFL
                   condition where Δ⁢t no longer depends on the mesh
                   size inside the locally refined region.},
  doi =           {10.1090/mcom/3650},
  issn =          {0025-5718, 1088-6842},
  language =      {en},
}

@article{CarleHochbruck:22:article:Error-Analysis,
  author =        {Carle, C. and Hochbruck, M.},
  journal =       {SIAM Journal on Numerical Analysis},
  month =         {10},
  number =        {5},
  pages =         {2897--2924},
  publisher =     {{Society for Industrial and Applied Mathematics}},
  title =         {Error Analysis of Multirate Leapfrog-Type Methods for
                   Second-Order Semilinear {ODEs}},
  volume =        {60},
  year =          {2022},
  abstract =      {In this paper we propose two exponential integrators
                   of first and second order applied to a class of
                   quasilinear wave-type equations. The analytical
                   framework is an extension of the classical Kato
                   framework and covers quasilinear Maxwell's equations
                   in full space and on a smooth domain as well as a
                   class of quasilinear wave equations. In contrast to
                   earlier works, we do not assume regularity of the
                   solution but only on the data. From this we deduce a
                   well-posedness result upon which we base our error
                   analysis. Compared to existing results, our error
                   bounds require less regularity in space and in time.
                   We include numerical examples to confirm our
                   theoretical findings.},
  doi =           {10.1137/21M1427255},
  issn =          {0036-1429},
}

@misc{Chaumont-FreletErn:24:misc:Damped-Energy-Norm,
  author =        {{Chaumont-Frelet}, T. and Ern, A.},
  month =         {03},
  number =        {arXiv:2403.12954},
  publisher =     {arXiv},
  title =         {Damped Energy-Norm a Posteriori Error Estimates for
                   Fully Discrete Approximations of the Wave Equation
                   Using {{C2-reconstructions}}},
  year =          {2024},
  abstract =      {We derive a posteriori error estimates for the the
                   scalar wave equation discretized in space by
                   continuous finite elements and in time by the
                   explicit leapfrog scheme. Our analysis combines the
                   idea of invoking extra time-regularity for the
                   right-hand side, as previously introduced in the
                   space semi-discrete setting, with a novel, piecewise
                   quartic, globally twice-differentiable
                   time-reconstruction of the fully discrete solution.
                   Our main results show that the proposed estimator is
                   reliable and efficient in a damped energy norm. These
                   properties are illustrated in a series of numerical
                   examples.},
  doi =           {10.48550/arXiv.2403.12954},
}

@techreport{Chaumont-FreletErn:24:techreport:Damped-Energy-Norm,
	abstract = {We derive a posteriori error estimates for the the scalar wave equation discretized in space by continuous finite elements and in time by the explicit leapfrog scheme. Our analysis combines the idea of invoking extra time-regularity for the right-hand side, as previously introduced in the space semi-discrete setting, with a novel, piecewise quartic, globally twice-differentiable time-reconstruction of the fully discrete solution. Our main results show that the proposed estimator is reliable and efficient in a damped energy norm. These properties are illustrated in a series of numerical examples.},
	archiveprefix = {arxiv},
	author = {{Chaumont-Frelet}, T. and Ern, A.},
	date-added = {2024-06-21 14:05:13 +0100},
	date-modified = {2025-05-07 08:48:21 +0100},
	doi = {10.48550/arXiv.2403.12954},
	eprint = {2403.12954},
	file = {/Users/ol20/Zotero/storage/BKWMKDAF/Chaumont-Frelet and Ern - 2024 - Damped energy-norm a posteriori error estimates fo.pdf;/Users/ol20/Zotero/storage/3RHRB8XA/2403.html},
	keywords = {Mathematics - Numerical Analysis},
	month = 03,
	number = {arXiv:2403.12954},
	primaryclass = {cs, math},
	publisher = {arXiv},
	title = {Damped Energy-Norm a Posteriori Error Estimates for Fully Discrete Approximations of the Wave Equation Using {{C2-reconstructions}}},
	year = {2024},
	bdsk-file-1 = {YnBsaXN0MDDSAQIDBFxyZWxhdGl2ZVBhdGhYYm9va21hcmtfEIAuLi8uLi9MaXRlcmF0dXJlL0F1dGhvci9DL0NoL0NoYXVtb250LUZyZWxldEVybi0yMDI0LUEtbWlzYy1EYW1wZWQgRW5lcmd5LU5vcm0gUG9zdGVyaW9yaSBFcnJvciBFc3RpbWF0ZXMgZm9yIEZ1bGx5IERpc2NyZXRlLnBkZk8RBORib29r5AQAAAAABBAwAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAADgAwAABQAAAAEBAABVc2VycwAAAAQAAAABAQAAb2wyMAcAAAABAQAARHJvcGJveAAKAAAAAQEAAExpdGVyYXR1cmUAAAYAAAABAQAAQXV0aG9yAAABAAAAAQEAAEMAAAACAAAAAQEAAENoAABjAAAAAQEAAENoYXVtb250LUZyZWxldEVybi0yMDI0LUEtbWlzYy1EYW1wZWQgRW5lcmd5LU5vcm0gUG9zdGVyaW9yaSBFcnJvciBFc3RpbWF0ZXMgZm9yIEZ1bGx5IERpc2NyZXRlLnBkZgAgAAAAAQYAAAQAAAAUAAAAIAAAADAAAABEAAAAVAAAAGAAAABsAAAACAAAAAQDAADrXAAAAAAAAAgAAAAEAwAAFG8EAAAAAAAIAAAABAMAAKXiKAAAAAAACAAAAAQDAABD5SgAAAAAAAgAAAAEAwAASOYoAAAAAAAIAAAABAMAAE7qKAAAAAAACAAAAAQDAACw8SgAAAAAAAgAAAAEAwAAAXibBQAAAAAgAAAAAQYAAAABAAAQAQAAIAEAADABAABAAQAAUAEAAGABAABwAQAACAAAAAAEAABBxhIW1OMHLxgAAAABAgAAAQAAAAAAAAAPAAAAAAAAAAAAAAAAAAAACAAAAAQDAAAGAAAAAAAAAAQAAAADAwAA5BQAAAgAAAABCQAAZmlsZTovLy8MAAAAAQEAAE1hY2ludG9zaCBIRAgAAAAEAwAAAJCClucAAAAIAAAAAAQAAEHGvNWFAAAAJAAAAAEBAAAzRUE1RjQzNC00RDc4LTQxQTQtQkQ1Ny05NDE1OTE1NENGOTEYAAAAAQIAAIEAAAABAAAA7xMAAAEAAAAAAAAAAAAAAAEAAAABAQAALwAAAAAAAAABBQAAQAEAAAECAAA2ZjM1NDE4ZWRjODc4YjkyMzg2M2ZmNjk4ZDc2Njg0MDc0NGI0ZDJlY2I2NmJiYWMyYjA2MDJiNjU2MGVkZDQxOzAwOzAwMDAwMDAwOzAwMDAwMDAwOzAwMDAwMDAwOzAwMDAwMDAwMDAwMDAwMjA7Y29tLmFwcGxlLmFwcC1zYW5kYm94LnJlYWQtd3JpdGU7MDE7MDEwMDAwMGY7MDAwMDAwMDAwNTliNzgwMTswMTsvdXNlcnMvb2wyMC9kcm9wYm94L2xpdGVyYXR1cmUvYXV0aG9yL2MvY2gvY2hhdW1vbnQtZnJlbGV0ZXJuLTIwMjQtYS1taXNjLWRhbXBlZCBlbmVyZ3ktbm9ybSBwb3N0ZXJpb3JpIGVycm9yIGVzdGltYXRlcyBmb3IgZnVsbHkgZGlzY3JldGUucGRmAMwAAAD+////AQAAAAAAAAAQAAAABBAAANgAAAAAAAAABRAAAIABAAAAAAAAEBAAALgBAAAAAAAAQBAAAKgBAAAAAAAAAiAAAIQCAAAAAAAABSAAAPQBAAAAAAAAECAAAAQCAAAAAAAAESAAADgCAAAAAAAAEiAAABgCAAAAAAAAEyAAACgCAAAAAAAAICAAAGQCAAAAAAAAMCAAAJACAAAAAAAAAcAAANgBAAAAAAAAEcAAABQAAAAAAAAAEsAAAOgBAAAAAAAAgPAAAJgCAAAAAAAAAAgADQAaACMApgAAAAAAAAIBAAAAAAAAAAUAAAAAAAAAAAAAAAAAAAWO},
	bdsk-file-2 = {YnBsaXN0MDDSAQIDBFxyZWxhdGl2ZVBhdGhYYm9va21hcmtfEIAuLi8uLi9MaXRlcmF0dXJlL0F1dGhvci9DL0NoL0NoYXVtb250LUZyZWxldEVybi0yMDI0LUItbWlzYy1EYW1wZWQgRW5lcmd5LU5vcm0gUG9zdGVyaW9yaSBFcnJvciBFc3RpbWF0ZXMgZm9yIEZ1bGx5IERpc2NyZXRlLnBkZk8RBORib29r5AQAAAAABBAwAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAAADgAwAABQAAAAEBAABVc2VycwAAAAQAAAABAQAAb2wyMAcAAAABAQAARHJvcGJveAAKAAAAAQEAAExpdGVyYXR1cmUAAAYAAAABAQAAQXV0aG9yAAABAAAAAQEAAEMAAAACAAAAAQEAAENoAABjAAAAAQEAAENoYXVtb250LUZyZWxldEVybi0yMDI0LUItbWlzYy1EYW1wZWQgRW5lcmd5LU5vcm0gUG9zdGVyaW9yaSBFcnJvciBFc3RpbWF0ZXMgZm9yIEZ1bGx5IERpc2NyZXRlLnBkZgAgAAAAAQYAAAQAAAAUAAAAIAAAADAAAABEAAAAVAAAAGAAAABsAAAACAAAAAQDAADrXAAAAAAAAAgAAAAEAwAAFG8EAAAAAAAIAAAABAMAAKXiKAAAAAAACAAAAAQDAABD5SgAAAAAAAgAAAAEAwAASOYoAAAAAAAIAAAABAMAAE7qKAAAAAAACAAAAAQDAACw8SgAAAAAAAgAAAAEAwAAY2WhBQAAAAAgAAAAAQYAAAABAAAQAQAAIAEAADABAABAAQAAUAEAAGABAABwAQAACAAAAAAEAABBxhLZFk2+gBgAAAABAgAAAQAAAAAAAAAPAAAAAAAAAAAAAAAAAAAACAAAAAQDAAAGAAAAAAAAAAQAAAADAwAA5BQAAAgAAAABCQAAZmlsZTovLy8MAAAAAQEAAE1hY2ludG9zaCBIRAgAAAAEAwAAAJCClucAAAAIAAAAAAQAAEHGvNWFAAAAJAAAAAEBAAAzRUE1RjQzNC00RDc4LTQxQTQtQkQ1Ny05NDE1OTE1NENGOTEYAAAAAQIAAIEAAAABAAAA7xMAAAEAAAAAAAAAAAAAAAEAAAABAQAALwAAAAAAAAABBQAAQAEAAAECAAAwZDYyYjMxYjNkYTFkNjQxNjE3YTI3Y2EyYzZhYmM2NGNmMmZiMWVlZTIzZTQwNDM2N2Q3ZjM2ZjdjZjc2NjkyOzAwOzAwMDAwMDAwOzAwMDAwMDAwOzAwMDAwMDAwOzAwMDAwMDAwMDAwMDAwMjA7Y29tLmFwcGxlLmFwcC1zYW5kYm94LnJlYWQtd3JpdGU7MDE7MDEwMDAwMGY7MDAwMDAwMDAwNWExNjU2MzswMTsvdXNlcnMvb2wyMC9kcm9wYm94L2xpdGVyYXR1cmUvYXV0aG9yL2MvY2gvY2hhdW1vbnQtZnJlbGV0ZXJuLTIwMjQtYi1taXNjLWRhbXBlZCBlbmVyZ3ktbm9ybSBwb3N0ZXJpb3JpIGVycm9yIGVzdGltYXRlcyBmb3IgZnVsbHkgZGlzY3JldGUucGRmAMwAAAD+////AQAAAAAAAAAQAAAABBAAANgAAAAAAAAABRAAAIABAAAAAAAAEBAAALgBAAAAAAAAQBAAAKgBAAAAAAAAAiAAAIQCAAAAAAAABSAAAPQBAAAAAAAAECAAAAQCAAAAAAAAESAAADgCAAAAAAAAEiAAABgCAAAAAAAAEyAAACgCAAAAAAAAICAAAGQCAAAAAAAAMCAAAJACAAAAAAAAAcAAANgBAAAAAAAAEcAAABQAAAAAAAAAEsAAAOgBAAAAAAAAgPAAAJgCAAAAAAAAAAgADQAaACMApgAAAAAAAAIBAAAAAAAAAAUAAAAAAAAAAAAAAAAAAAWO},
	bdsk-url-1 = {https://doi.org/10.48550/arXiv.2403.12954}}

@article{Chaumont-Frelet:23:article:Asymptotically-Constant-Free,
  author =        {{Chaumont-Frelet}, T.},
  journal =       {SIAM Journal on Scientific Computing},
  month =         {08},
  number =        {4},
  pages =         {A1591-A1620},
  publisher =     {{Society for Industrial and Applied Mathematics}},
  title =         {Asymptotically {{Constant-Free}} and
                   {{Polynomial-Degree-Robust}} a {{Posteriori
                   Estimates}} for {{Space Discretizations}} of the
                   {{Wave Equation}}},
  volume =        {45},
  year =          {2023},
  abstract =      {.We propose a new residual-based a posteriori error
                   estimator for discontinuous Galerkin discretizations
                   of time-harmonic Maxwell's equations in first-order
                   form. We establish that the estimator is reliable and
                   efficient, and the dependency of the reliability and
                   efficiency constants on the frequency is analyzed and
                   discussed. The proposed estimates generalize similar
                   results previously obtained for the Helmholtz
                   equation and conforming finite element
                   discretizations of Maxwell's equations. In addition,
                   for the discontinuous Galerkin scheme considered
                   here, we also show that the proposed estimator is
                   asymptotically constant-free for smooth solutions.},
  doi =           {10.1137/22M1485619},
  issn =          {1064-8275},
}

@article{CohenJolyRobertsTordjman:01:article:Higher-Order,
  author =        {Cohen, G. and Joly, P. and Roberts, J. E. and
                   Tordjman, N.},
  journal =       {SIAM Journal on Numerical Analysis},
  month =         {01},
  number =        {6},
  pages =         {2047--2078},
  publisher =     {{Society for Industrial and Applied Mathematics}},
  title =         {Higher {{Order Triangular Finite Elements}} with
                   {{Mass Lumping}} for the {{Wave Equation}}},
  volume =        {38},
  year =          {2001},
  abstract =      {We construct and analyze a new family of rectangular
                   (two-dimensional) or cubic (three-dimensional) mixed
                   finite elements for the approximation of the acoustic
                   wave equations. The main advantage of this element is
                   that it permits us to obtain through mass lumping an
                   explicit scheme even in an anisotropic medium.
                   Nonclassical error estimates are given for this new
                   element.},
  doi =           {10.1137/S0036142997329554},
  issn =          {0036-1429},
}

@article{LakkisMakridakis:06:article:Elliptic,
  author =        {Lakkis, O. and Makridakis, C.},
  journal =       {Math. Comp.},
  number =        {256},
  pages =         {1627--1658},
  title =         {Elliptic reconstruction and a posteriori error
                   estimates for fully discrete linear parabolic
                   problems},
  volume =        {75},
  year =          {2006},
  doi =           {10.1090/S0025-5718-06-01858-8},
  issn =          {0025-5718},
  url =           {https://doi.org/10.1090/S0025-5718-06-01858-8},
}

@article{DiazGrote:15:article:Multi-Level-Explicit,
  author =        {Diaz, J. and Grote, M. J.},
  journal =       {Comp. Meth. in Appl. Mech. Engin.},
  pages =         {240--265},
  title =         {Multi-Level Explicit Local Time-Stepping Methods for
                   Second-Order Wave Equations},
  volume =        {291},
  year =          {2015},
  abstract =      {Local mesh refinement severely impedes the efficiency
                   of explicit time-stepping methods for numerical wave
                   propagation. Local time-stepping (LTS) methods
                   overcome the bottleneck due to a few small elements
                   by allowing smaller time-steps precisely where those
                   elements are located. Yet when the region of local
                   mesh refinement itself contains a sub-region of even
                   smaller elements, any local time-step again will be
                   overly restricted. To remedy the repeated bottleneck
                   caused by hierarchical mesh refinement, multi-level
                   local time-stepping methods are proposed, which
                   permit the use of the appropriate time-step at every
                   level of mesh refinement. Based on the LTS methods
                   from Diaz and Grote (2009), these multi-level LTS
                   methods are explicit, yield arbitrarily high accuracy
                   and conserve the energy. Numerical experiments
                   illustrate the theoretical properties and the
                   usefulness of these methods.},
  doi =           {10.1016/j.cma.2015.03.027},
  issn =          {0045-7825},
}

@book{Braess:07:book:Finite,
  address =       {Cambridge},
  author =        {Braess, D.},
  edition =       {3},
  month =         {04},
  publisher =     {Cambridge University Press},
  title =         {Finite elements: theory, fast solvers, and
                   applications in elasticity theory},
  year =          {2007},
  doi =           {10.1017/CBO9780511618635},
  isbn =          {978-0-511-61863-5},
  url =           {http://www.worldcat.org/oclc/776966850},
}

@article{BraessPillweinSchoberl:09:article:Equilibrated,
  author =        {Braess, D. and Pillwein, V. and
                   Sch{\"o}berl, J.},
  journal =       {Computer Methods in Applied Mechanics and
                   Engineering},
  month =         {03},
  number =        {13-14},
  pages =         {1189--1197},
  title =         {Equilibrated residual error estimates are p-robust},
  volume =        {198},
  year =          {2009},
  doi =           {10.1016/j.cma.2008.12.010},
  issn =          {00457825},
  language =      {en},
}

@article{BabuskaRheinboldt:78:article:Error,
  author =        {{Babu{\v s}ka}, I. and Rheinboldt, W. C.},
  journal =       {SIAM Journal on Numerical Analysis},
  number =        {4},
  pages =         {736--754},
  title =         {Error estimates for adaptive finite element
                   computations},
  volume =        {15},
  year =          {1978},
  annote =        {old MR number: 58 \#3400 MR reviewer: William W.
                   Hager MR class: 65J05 (65N30)},
  doi =           {10.1137/0715049},
  issn =          {0036-1429},
  url =           {https://mathscinet.ams.org/mathscinet-getitem?mr=483395},
}
@article {CarleHochbruck:24:article:Error,
    AUTHOR = {Carle, C. and Hochbruck, M.},
     TITLE = {Error analysis of second-order local time integration methods
              for discontinuous {G}alerkin discretizations of linear wave
              equations},
   JOURNAL = {Math. Comp.},
  FJOURNAL = {Mathematics of Computation},
    VOLUME = {93},
      YEAR = {2024},
    NUMBER = {350},
     PAGES = {2611--2641},
      ISSN = {0025-5718,1088-6842},
   MRCLASS = {65M12 (65M15 65M20 65M22 65M60)},
  MRNUMBER = {4780340},
       DOI = {10.1090/mcom/3952},
       URL = {https://doi.org/10.1090/mcom/3952},
}
@misc{GroteMichelSauter:24:ExplicitLocalTimeSteppingInhomogeneous,
      title={Explicit Local Time-Stepping for the Inhomogeneous Wave Equation with Optimal Convergence}, 
      author={Grote, M. J. and Michel, S. and Sauter, S. A.},
      year={2024},
      eprint={2409.18085},
      archivePrefix={arXiv},
      primaryClass={math.NA},
      url={https://arxiv.org/abs/2409.18085}, 
}
@misc{GroteLakkisSantos:24:PosterioriErrorEstimatesWave,
      title={A posteriori error estimates for the wave equation with mesh change in the leapfrog method}, 
      author={Grote, M. J. and Lakkis, O. and Santos, C.},
      year={2024},
      eprint={2411.16933},
      archivePrefix={arXiv},
      primaryClass={math.NA},
      url={https://arxiv.org/abs/2411.16933}, 
}
@article{Rietmann:17:NewmarkLocalTime,
title = {Newmark local time stepping on high-performance computing architectures},
journal = {Journal of Computational Physics},
volume = {334},
pages = {308-326},
year = {2017},
issn = {0021-9991},
doi = {https://doi.org/10.1016/j.jcp.2016.11.012},
url = {https://www.sciencedirect.com/science/article/pii/S0021999116305988},
author = {Rietmann, M. and Grote, M. and Peter, D. and Schenk, O.},
keywords = {Seismic wave propagation, Local-time stepping, Multi-rate time stepping},
abstract = {In multi-scale complex media, finite element meshes often require areas of local refinement, creating small elements that can dramatically reduce the global time-step for wave-propagation problems due to the CFL condition. Local time stepping (LTS) algorithms allow an explicit time-stepping scheme to adapt the time-step to the element size, allowing near-optimal time-steps everywhere in the mesh. We develop an efficient multilevel LTS-Newmark scheme and implement it in a widely used continuous finite element seismic wave-propagation package. In particular, we extend the standard LTS formulation with adaptations to continuous finite element methods that can be implemented very efficiently with very strong element-size contrasts (more than 100x). Capable of running on large CPU and GPU clusters, we present both synthetic validation examples and large scale, realistic application examples to demonstrate the performance and applicability of the method and implementation on thousands of CPU cores and hundreds of GPUs.}
}
@book{LionsMagenes:72:.Non-HomogeneousBoundaryValueProblemsandApplications,
  author =        {J. Lions and E. Magenes},
  publisher =     {Springer-Verlag},
  title =         {Non-Homogeneous Boundary Value Problems
and Applications},
  year =          {1972}
}

@book{SchmidtSiebert:05:book:Design,
	address = {Berlin},
	author = {Schmidt, A. and Siebert, K. G.},
	date-added = {2016-01-21 16:37:08 +0000},
	date-modified = {2025-06-06 08:22:49 +0100},
	doi = {10.1007/b138692},
	isbn = {3-540-22842-X},
	keywords = {adaptive, mesh, refinement, partial differential equation, differential equation, analysis, computational, C, programming},
	mrclass = {65-02 (65-04 65N30 65N50 68P05)},
	mrnumber = {MR2127659},
	note = {The finite element toolbox ALBERTA, With 1 CD-ROM (Unix/Linux)},
	pages = {xii+315},
	publisher = {Springer-Verlag},
	series = {Lecture Notes in Computational Science and Engineering},
	title = {Design of adaptive finite element software},
	url = {http://www.worldcat.org/oclc/488984204},
	volume = {42},
	year = {2005}}
@misc{ferrari2025intrinsicunconditionalstabilityspacetime,
      title={Intrinsic unconditional stability in space-time isogeometric approximation of the acoustic wave equation in second-order formulation}, 
      author={Ferrari,M. and Perugia,I.},
      year={2025},
      eprint={2503.11166},
      archivePrefix={arXiv},
      primaryClass={math.NA},
      url={https://arxiv.org/abs/2503.11166}, 
}
@techreport{Chen:2008ifem,
	author = {Chen, L.},
	journal = {Technical Report, University of California at Irvine},
	title = {{$i$FEM}: an integrated finite element methods package in {MATLAB}},
	url = {https://github.com/lyc102/ifem},
	year = {2009}}
